FairTraDEX: A Decentralised Exchange Preventing Value Extraction

We present FairTraDEX, a decentralized exchange (DEX) protocol based on frequent batch auctions (FBAs), which provides formal game-theoretic guarantees against extractable value. FBAs when run by a trusted third-party provide unique game-theoretic optimal strategies which ensure players are shown prices equal to the liquidity provider's fair price, excluding explicit, pre-determined fees. FairTraDEX replicates the key features of an FBA that provide these game-theoretic guarantees using a combination of set-membership in zero-knowledge protocols and an escrow-enforced commit-reveal protocol. We extend the results of FBAs to handle monopolistic and/or malicious liquidity providers. We provide real-world examples that demonstrate that the costs of executing orders in existing academic and industry-standard protocols become prohibitive as order size increases due to basic value extraction techniques, popularized as maximal extractable value. We further demonstrate that FairTraDEX protects against these execution costs, guaranteeing a fixed fee model independent of order size, the first guarantee of it's kind for a DEX protocol. We also provide detailed Solidity and pseudo-code implementations of FairTraDEX, making FairTraDEX a novel and practical contribution.

==> Appendices/ProtocolFlow.tex <==
\newpage

\section{Protocol Flow}\label{app:ProtocolFlow}

Client Protocol Flow: \\

\begin{center}
\scalebox{0.5}{
$\begin{array}{c c c}
    \text{\textsf{Client}} \ \client & & \protocolContract \\
    \hline
    \hline
    & \textbf{Register} & \\
    \commSerialNum, \commRandomness \gets \text{genZKInfo}() & &  \\
    \regToken \assign \commit(\commSerialNum, \commRandomness) & &  \\
    & \underset{\bitcoin: \ \escrowClient+ \feeRelayer}{\xrightarrow{\hspace{1em}  \ \regToken \hspace{1em}}} &  \\
    & & \clients\getAppend(\regToken) \\
    \hline
     & \textbf{Commit} & \\
    \token \in \{\tokenA, \tokenB\}& & \\
    \tokenAmount \in \mathbb{R}_{>0}& & \\
    \tokenPrice \in \mathbb{R}_{>0} \cup \{\marketOrder\}& & \\
    \width \in \mathbb{R}_{\geq 1}& & \\
    \commitment \gets \commit(\token, \tokenAmount, \tokenPrice, \width) & &\\
    \proofZK \gets \text{genZKProof}(\regToken, \clients,*) & &  \\
    & \xrightarrow{\hspace{1em} \relay(\tagClientCommit, \commitment, \commSerialNum, \proofZK) \hspace{1em}}& \\
    &  & \clientCommits\getAppend([\commSerialNum,\commitment]) \\
    \hline
     & \textbf{Reveal} &  \\
    \text{leave} \in \{0,1\}& &   \\
    \commSerialNum', \commRandomness' \gets
    \begin{cases}
    \begin{array}{l l}
    \varnothing, & \text{if}\ \text{leave}=1 \\
    \text{genZKInfo}(), & \text{if}\ \text{leave}=0
    \end{array}
    \end{cases} 
    & & \\
    \regTokenNew \gets
    \begin{cases}
    \begin{array}{l l}
    \varnothing, & \text{if}\ \text{leave}=1 \\
    \commit(\commSerialNum', \commRandomness'), & \text{if}\ \text{leave}=0
    \end{array}
    \end{cases} 
    & & \\
    & \underset{\begin{array}{l l}
    \tokenA: \ \textit{minimum}(\tokenAmount, \tokenAMaxSizeClient), & \text{if}\ \token =\tokenA \\
    \tokenB: \ \textit{minimum}(\tokenAmount, \tokenBMaxSizeClient), & \text{if}\ \token =\tokenB \\
    \bitcoin: \ \feeRelayer, & \text{if} \ \regTokenNew = \varnothing
    \end{array}}{\xrightarrow{\hspace{1em}
     : \ \tagClientReveal,\token, \tokenAmount, \width, \tokenPrice, \ \commSerialNum, \commRandomness, \regToken, \regTokenNew 
    \hspace{1em}}}  & \\
    & & \revealedOrders\getAppend([\client, \token, \tokenAmount,  \tokenPrice, \width])  \\
    &  & \clients\remove(\regToken) \\
    & & \clientCommits\remove(\commSerialNum)\\
    & & \clients\getAppend(\regTokenNew), \ \text{if}\ \regTokenNew \neq \varnothing \\
    & \underset{\bitcoin: \ \feeRelayer \ \text{if} \ \regTokenNew=\varnothing}{\xrightarrow{\hspace{6em}}} & \\
    & \underset{\bitcoin: \ \escrowClient \ \text{if} \ \regTokenNew=\varnothing}{\xleftarrow{\hspace{6em}}} & \\
    \hline
     & \textbf{Resolution} & \\
    & & \clearingPrice \assign \textit{getClearingPrice}(\revealedOrders) \\
    & & \tokenTradeSize \assign \textit{getClearingVolume}(\clearingPrice, [\token, \tokenAmount,  \tokenPrice, \width], \revealedOrders)\\
    &  \underset{\begin{array}{l l}
    \tokenB: \ \tokenTradeSize, & \text{if}\ \token =\tokenA, \\
    \tokenA: \ \tokenTradeSize, & \text{if}\ \token =\tokenB .
    \end{array}}{\xleftarrow{\hspace{6em} }} & \\
    & & \textit{leftovers} \assign \begin{cases}
    \begin{array}{l l}
    \tokenAmount- \frac{\tokenTradeSize}{\clearingPrice}, & \text{if}\ \token = \tokenA \\
    \tokenAmount- (\tokenTradeSize \cdot \clearingPrice), & \text{if}\ \token = \tokenB
    \end{array}
    \end{cases}  \\
    & \underset{\begin{array}{l l}
    \tokenA: \ \textit{leftovers}, & \text{if}\ \token =\tokenA, \\
    \tokenB: \ \textit{leftovers}, & \text{if}\ \token =\tokenB.
    \end{array}}{\xleftarrow{\hspace{6em} }} & \\
    \hline
    \end{array}$}    
\end{center}

MM Protocol Flow: \\
\\

\scalebox{0.55}{
$\begin{array}{c c c}
    \protocolContract & & \text{\textsf{Market Maker}} \ \MM \\
    \hline
    \hline
    & \textbf{Commit} & \\
    & & \MMBidPrice  \in \mathbb{R}_{>0} \\
    & &  \MMBidAmount \in \mathbb{R}_{>0} \\
    & & \MMOfferPrice  \in \mathbb{R}_{>0} \\
    & & \MMOfferAmount  \in \mathbb{R}_{>0} \\
    & & \commitment \gets \commit(\MMBidPrice, \ \MMBidAmount, \ \MMOfferPrice,  \ \MMOfferAmount)  \\
    & \underset{\bitcoin: \ \escrowMM}{\xleftarrow{\hspace{1em} \
    \tagMMCommit, \commitment 
    \hspace{1em}}} & \\
    \MMCommits\getAppend([\MM, \commitment])& & \\
    \hline \\
    & \textbf{Reveal} &  \\
    & &  \\
    & \underset{\bitcoin: \ \escrowMM}{\xrightarrow{\hspace{6em}}}  & \\
    & & x \assign  \textit{minimum}(\MMBidAmount, \tokenAMaxSizeClient)   \\
    & & y \assign  \textit{minimum}(\MMOfferAmount, \tokenBMaxSizeClient) \\
    & \underset{\tokenA: \ x, \ \tokenB: \ y }{\xleftarrow{\hspace{1em}  \ \tagMMReveal,\MMBidPrice, \ \MMBidAmount, \ \MMOfferPrice,  \ \MMOfferAmount \hspace{1em}}}  & \\
    \tightestWidth \assign \frac{\MMOfferPrice}{\MMBidPrice}, \ \text{if} \ \big( \frac{\MMOfferPrice}{\MMBidPrice}<\tightestWidth \ \logicalOr \ \tightestWidth = \any \big) & & \\
    \revealedOrders\getAppend([ \MM, \tokenA, x,  \MMBidPrice, \any ]) & & \\
    \revealedOrders\getAppend([ \MM, \tokenB,  y,  \MMOfferPrice, \any ]) & & \\
    \MMCommits\remove(\MM) & & \\
    \hline
     & \textbf{Resolution} & \\
     \clearingPrice \assign \textit{getClearingPrice}(\revealedOrders) & & \\
    \tokenTradeSize_B \assign \textit{getClearingVolume}(\clearingPrice, [ \tokenA,  x,  \MMBidPrice, \any], \revealedOrders) & & \\
    \textit{bidLeftovers} \assign x - \frac{\tokenTradeSize_A}{\clearingPrice} & &  \\
    \tokenTradeSize_A \assign \textit{getClearingVolume}(\clearingPrice, [ \tokenB,  y,  \MMOfferPrice, \any], \revealedOrders) & & \\
    \textit{offerLeftovers} \assign y - (\tokenTradeSize_A \cdot \clearingPrice) & &  \\
    & \underset{\begin{array}{l l}
    \tokenA: \ \tokenTradeSize_A + \ \textit{bidLeftovers} \\
    \tokenB: \ \tokenTradeSize_B + \ \textit{offerLeftovers}.
    \end{array}}{\xrightarrow{\hspace{6em} }} & \\
    & & \\
    \hline
    \end{array}$}


==> AttacksCESC.tex <==
\section{Cost-Benefit Analysis of \texorpdfstring{$\protocolName$}{TEXT}}\label{sec:Attacks}

The aim of this section is to demonstrate the contributory significance of FairTra-DEX vs. current state-of-the-art protocols as introduced in Section \ref{sec:RelatedWork}.
In Table \ref{table:RelatedWorkComparison} we include an overview of the gas costs for running $\protocolName$ compared to the previous blockchain-based attempts to implement batch auctions of \cite{PubliclyVerifiableSecrecyPreservingPeriodicAuctionsGalal,BlockAuctionPeriodicAuctionsConstantinides}, with numbers taken from the respective papers. It can be seen that $\protocolName$ has a slightly greater upfront gas cost for clients, but a lesser cost for MMs. 

To demonstrate the benefits of $\protocolName$, Table \ref{table:AttackComparison} compares specific swaps that allow for EEV attacks in existing state-of-the-art protocols. 
We perform our analysis on ETH/USDC swaps, as this is the highest volume pool on Uniswap, which at time of writing had pool sizes of 120k ETH and 185M USDC, an indicative MIFP of 1 ETH equal to 1,540 USDC \cite{UniswapWebsite}. Furthermore, we use a gas cost of 7 gwei \cite{ETHGasCost}. 

Consider 3 buy ETH orders of 10k, 500k and 10M USDC from 2 different players who are known to need to trade at any price. $\player_1$ has large quantities of both ETH and USDC, and buys or sells ETH pseudo-randomly, while $\player_2$ only owns USDC/only buys ETH. We take the estimated impact for each order to be $~0$, $0.15\%$  and $1\%$ respectively, numbers taken from the Uniswap V3 API \cite{UniswapWebsite} (these are more realistic impacts than those implied by the constant product impact \cite{AnalysisOfUniswapAngeris} of $~0$, $0.54\%$  and $11.1\%$ respectively, using starting pool sizes of ). Although this is a simplification of order impact, true impact is likely some multiple/factor of this impact. Protocol fees incentivizing MMs to provide liquidity are omitted as they are not considered in the provided academic protocols. After gas costs, this fee should be approximately equal for all protocols (the Uniswap fee for this pool is $0.3\%$).


When $\player_1$ submits an order in $\protocolName$ or \cite{PubliclyVerifiableSecrecyPreservingPeriodicAuctionsGalal}, no information is gained about the direction of the trade. However, in \cite{BlockAuctionPeriodicAuctionsConstantinides}, direction is revealed. As such, any blockchain participant can front run that impact on all other markets, and thus the MIFP for any MM responding to the order will be the impacted MIFP. When $\player_2$ submits an order in either of \cite{BlockAuctionPeriodicAuctionsConstantinides,PubliclyVerifiableSecrecyPreservingPeriodicAuctionsGalal} the direction is known, and the MIFP is impacted in the same way as for $\player_1$, \textbf{before} any player interacts with $\player_2$, giving $\player_2$ a worse price. Using estimated price impacts of $~0$, $0.15\%$  and $1\%$, Table \ref{table:AttackComparison} demonstrates the costs of executing these swaps, excluding transaction fees, in these protocols, and Uniswap. For Uniswap, we must also add the recommended slippage, an additional $0.5\%$ of the order size, as it is always in a block producers interest to give Uniswap players worst execution. It can be seen that these costs become increasingly more significant as order size increases, dominating the differences in gas costs of Table \ref{table:RelatedWorkComparison}.  




Although Table \ref{table:AttackComparison} can be seen as simplifying how orders are handled, it demonstrates two crucial motivators for our work. Firstly, any information revealed about clients before a trade is agreed can, is and will continue to be used against clients. Furthermore, this cost is not necessarily paid to the MM. As orders are committed in public, any blockchain participant can use the committed information to front run the impact on the MIFP before the client or MM has an opportunity to trade, extracting money from the DEX protocol. Secondly, as the effects of these value-extraction techniques increase super-linearly in order-size, a protocol with the value-extraction guarantees of $\protocolName$ is needed to allow typically large clients to utilise the benefits of DEXs, and blockchain protocols in as a whole, at a fixed cost, as demonstrated in Table \ref{table:RelatedWorkComparison}, without incurring the prohibitive execution costs of previous solutions, as demonstrated in Table \ref{table:AttackComparison}.

\vspace{-0.4cm}

\begin{table*}[h]
\centering
\begin{tabular}{l|c|c|c|c}
    \toprule
     & $\protocolName$ \footnotemark  & Uniswap & \cite{BlockAuctionPeriodicAuctionsConstantinides} & \cite{PubliclyVerifiableSecrecyPreservingPeriodicAuctionsGalal} \\
    \midrule
    Register & 112,800 & -  & 87,000 & -  \\  
    Commit Client & 344,500 & -  & 52,000 & 276,150  \\ 
    Commit MM (per order) & 24,300 & -   & 52,000 & 276,150 \\  
    Reveal (per order) & 172,000 & 190,000  & 171,000 & 48,750 \\  
    Settle (per order) \footnotemark   & 45,500 & -  & 122,500 & 54,000  \\ 
    \midrule
    Total Client  & 674,800 & 190,000 & 432,500 & 378,900 \\
    Total MM & 266,100  & -    & 397,500 & 649,050 \\
    \midrule
    Total Client (USDC) & 7.27 & 2.05 & 4.66 & 4.08 \\
    Total MM (USDC) & 2.87 & - & 4.09 & 7 \\
    \bottomrule
  \end{tabular}
  \caption{Comparison of gas costs in batch-auction implementations\label{table:RelatedWorkComparison}.
  \footnotesize{\textsuperscript{2} Costs provided for $\protocolName$ are amortised over 128 client orders and 8 markets. \textsuperscript{3} We add an estimated cost for token transfer from smart contract to player of 40,000 to the figures provided in \cite{PubliclyVerifiableSecrecyPreservingPeriodicAuctionsGalal} to standardise the costs therein with those of $\protocolName$ and \cite{BlockAuctionPeriodicAuctionsConstantinides}.} }
\end{table*}


\vspace{-1.8cm}

\begin{table*}[h]
\centering
\begin{tabular}{l|c|c|c|c}
    \toprule
     & $\protocolName$  & Uniswap & \cite{BlockAuctionPeriodicAuctionsConstantinides} & \cite{PubliclyVerifiableSecrecyPreservingPeriodicAuctionsGalal}  \\
    \midrule
    $\player_1$-10,000 & 0 & 50 & 0 & 0  \\
    $\player_2$-10,000 & 0 & 50 & 0 & 0 \\
    $\player_1$-500,000 & 0 & 3000 & 750 & 0 \\
    $\player_2$-500,000 & 0 & 3000 & 750 & 750 \\
    $\player_1$-10,000,000 & 0 & 150,000 & 100,000 & 0  \\
    $\player_2$-10,000,000 & 0 & 150,000 & 100,000 & 100,000 \\ 
    \bottomrule
  \end{tabular}
  \caption{Comparison of execution costs in USDC of batch-auction implementations. \label{table:AttackComparison}}
\end{table*}

\vspace{-1cm}

==> Thoughts.tex <==


Although AMMs have less message complexity, they have significant opportunity costs and risks, such as the opportunity cost of locked capital and impermanent loss, that do not occur $\protocolName$ or other 2-player exchange protocols. The \textit{total value locked} (TVL) in current DEX protocols according to DeFi Pulse\footnote{\url{https://defipulse.com/} Accessed: 20/10/2021} is $\$ 30$ billion. Compare this to an extreme capital requirement of 10 times the maximum allowed notional of an order based on current MIFP as escrow. According to CoinGecko\footnote{\url{https://www.coingecko.com/en/dex} Accessed: 20/10/2021}, the daily DEX volume is $\$ 4.7$ billion. Amortized per minute (an estimate for the time needed to complete a $\protocolName$ exchange), $\protocolName$ would require on average $10 \frac{\$4.7\textit{B}}{1440}=\$ 33$ million TVL, approximately 1000 times less than that of current DEXs.  




\subsection{DEX Value Extraction Attacks}

In this section we analyse the main value extraction attack techniques that plague DEXs. These are \textit{transaction omission}, \textit{transaction reordering}, \textit{selective participation}, and \textit{transaction injection}. For each attack we describe the strategy from the value extractor, which can be any of the block producer, the MM or the client. We first demonstrate how $\protocolName$ defends against such attacks, then analyse previous state-of-the-art protocols under these attacks in our Threat Model (Section \ref{sec:ThreatModel}). In the following, when considering a player $\playeri$ at phase $\phase$ of a protocol, let the set of all possible valid protocol transactions not already sent to the blockchain from other players for phase $\phase$ be $\transactionsPhase$. The following are the four \textit{proofness properties}.

\begin{enumerate}
    \item A protocol is \textit{transaction omission proof} if any protocol transaction submitted at the beginning of a protocol phase is committed to the blockchain during that phase.
    
    \item A protocol is \textit{selective participation proof} if following the protocol strategy has strictly greater expected value than not following the protocol strategy.
    
    \item A protocol is \textit{transaction reordering proof} if for any rational player $\playeri$ at phase $\phase$ and any $\tx \in \transactionsPhase$, it holds that for any $\playeri$ phase $\phase$ protocol transaction $\tx_i$, $E(\tx_i | \tx_i \textit{ exec. before } \tx)$ $ = E(\tx_i | \tx \textit{ exec. before } \tx_i)$.
    
    \item  A protocol is \textit{transaction injection proof} if:
    \begin{itemize}
        \item It is transaction reordering proof.
        
        \item For any rational player $\player_i$ at phase $\phase$ of a protocol, there is no subset of transactions $\{ \tx_1, ..., \tx_n\}$ $ \subseteq \transactionsPhase$, such that there exists a $\player_i$ phase $\phase$ protocol transaction $\tx_i$ with $E(\tx_i | $ $\{\tx_1, ..., \tx_n\}) \geq E(\tx_i )$ and $E(\tx_j | $ $\tx_i, \{\tx_1 ..., \tx_n\}\backslash \{ \tx_j\}) < E(\tx_j)$, for some $j \in \{1,...,n\}$.
    \end{itemize} 

\end{enumerate}

\begin{definition}
    A protocol is \textit{extractable value proof} if all four proofness properties hold. 
\end{definition}

\begin{theorem}
    $\protocolName$ is extractable value proof.
\end{theorem}

\begin{proof}
    In the following, we let the player $\playeri$ be rational, and use the fact that $\playeri$ assumes all other players are rational (Definition \ref{def:PlayerModel}). 
    \begin{enumerate}
        \item In our Threat Model we assume there is an upper bound $\revealTXDelay$ on the number of blocks required to commit a transaction to the blockchain. We analyse all protocols under this assumption. As such, every DEX can avail of $\revealTXDelay$ to ensure all protocol transactions are committed to the blockchain, nullifying transaction omission attacks. That is to say, $\protocolName$ is transaction omission proof.
        
        \item In Section \ref{sec:protocolIsWTT}, we demonstrate that all rational players who enter $\protocolName$ follow the protocol, which is to say, $\protocolName$ is selective participation proof. 
        
        \item It can be seen that the ordering of Request, Response and Reveal transactions within their respective phases does not affect their expected value in $\protocolName$. The expected value of a fixed set of transactions to be included in the Request phase depend only on transactions in the Response phase, and vice versa. The value of transactions to be included in the Reveal phase is fixed after the Response phase. Therefore, $\protocolName$ is transaction reordering proof.
        
        \item The argument for $\protocolName$ being transaction injection proof is a little more involved. To do this, we show that if there exists a $\playeri$ protocol transaction $\tx_i$ and $\{ \tx_1, ..., \tx_n\}$ $ \subseteq \transactionsPhase$ with $E(\tx_i | $ $\{\tx_1, ..., \tx_n\}) > E(\tx_i )$, then $E(\tx_j | $ $\tx_i, \{\tx_1 ..., \tx_n\}\backslash \{ \tx_j\}) > E(\tx_j)$ for all $j \in \{1,..,n\}$. As phases are run one at a time, when analysing each phase, only transactions from that phase are considered, as others are invalid.

        \begin{itemize}
            \item Request: In the case of a single client request per Request phase (each request initialises a unique instance of $\protocolName$), the Request phase is trivially transaction injection proof. 
            
            Consider instead the case where many requests can be included per Request phase. For a $\playeri$ Response transaction $\tx_i$, $\playeri$ can choose to add as many transactions from $\transactionsRequest$ as desired to increase the expected value of $\tx_i$. Consider the effect of adding a subset of transactions $\{ \tx_1, ..., \tx_n\}$ $ \subseteq \transactionsRequest$. We know Request transactions give no information about client direction, so adding client requests does not change the reference prices provided by rational MMs (Lemma \ref{lem:WTTMMstrat}). 
    
            If the expected width of rational MM markets is increasing (although not necessarily strictly) in the number of client requests, this implies the expected fee is increasing in the number of requests. Specifically, for a $\playeri$ Request transaction $\tx_i$ and any $\{ \tx_1, ..., \tx_n\}$ $ \subseteq \transactionsPhase$, it is the case that $E(\tx_i | $ $\{\tx_1, ..., \tx_n\}) \leq E(\tx_i )$. In this case, the Request phase is transaction injection proof. 
        
            If instead the expected MM widths are strictly decreasing in the number of requests\footnote{Which of these rational MM strategies is used in reality is beyond the scope of the paper.}, the expected fee for $\tx_i$ decreases, and the expected value of $\tx_i$ increases. If the expected fee strictly decreases for one request, it strictly decreases for all requests. This again implies transaction injection proof. Therefore, the Request phase is transaction injection proof.   
    
            \item Response: $\playeri$ can choose to add as many Response transactions from $\transactionsResponse$ as desired to increase the expected value of a $\playeri$ Response transaction $\tx_i$. We know Response transactions give no information about reference price or width. Consider the effect of adding another Response transaction $\tx' \in \transactionsResponse$. If the width of the market being committed in $\tx'$ is smaller than that in $\tx$, $\playeri$ loses the opportunity to trade, otherwise nothing changes. This is strictly dominated by not adding $\tx'$. Therefore, the Response phase is transaction injection proof. 
    
            \item Reveal: We know that the only valid Reveal transactions correspond to previously committed Request or Response transactions. As such $\transactionsReveal$ is empty, which trivially implies the Reveal phase is transaction injection proof.
        \end{itemize}
        This implies $\protocolName$ is transaction injection proof, and therefore extractable value proof.
    \end{enumerate}

\end{proof}



We now briefly outline the some of the attacks which the state-of-the-art protocols do not protect against. These protocols, and their vulnerabilities, are presented alongside $\protocolName$ in Table \ref{table:RelatedWorkComparison}.

\subsubsection{FairMM}

FairMM \cite{FairMMCiampi} is vulnerable to selective participation as there is no requirement for the MM to complete the protocol after seeing the clients order size and direction. Once a client reveals this information, the MM can update her valuation for the exchange price, front-running MMs and clients in other exchanges and/or only trading with the original client if the price goes against the client (a fundamental price indicator/the market disagrees with the client).

\subsubsection{P2DEX}

P2DEX \cite{P2DEXBaum} is vulnerable to selective participation in the case where one player controls a majority of the servers in the MM protocol. If one player controls all of the servers, the protocol is vulnerable to all of our attacks as the player controlling the MM protocol can learn all client order information. Furthermore, in \cite{P2DEXBaum} the authors instead assume that many players run the MM protocol, of which one is honest-by-default. Honesty is not a realistic assumption in decentralised protocols, and is not considered in the ByRa model. 

\subsubsection{Publicly Veriﬁable and Secrecy Preserving Periodic Auctions}

The protocol in \cite{PubliclyVerifiableSecrecyPreservingPeriodicAuctionsGalal} is vulnerable to injection attacks. By injecting many sell orders, the expected price at which a player's buy order gets filled decreases, which strictly increases the expectancy of a buy order. 

Practically, after clients submit orders in \cite{PubliclyVerifiableSecrecyPreservingPeriodicAuctionsGalal}, the final block producer gets to observe the number of buyers and sellers, which also implies an expected price at which trades occur. If the producer has a fair price which differs to the expected trading price based on the numbers of buyers and sellers, the producer can pay less/sell higher than their fair price (based on this expected trade price), extracting value from clients. 
Furthermore, the authors do not handle how a deposit is privately paid to the protocol contract in Ethereum. It is non-trivial to send tokens without the leakage of information about client identity/trade size/direction/impact. This further adds to the MEV available due to transaction injection in the order submission phase. 

\subsubsection{Automated Market Makers}

The vulnerabilities of AMMs have been well documented \cite{FlashBoys2.0}. Under our attack definitions, the most obvious vulnerability is to transaction reordering (which implies transaction injection). If the block producer is the sole liquidity provider of an AMM pool, the protocol is also vulnerable to selective participation. 
